UFNRec: Utilizing False Negative Samples for Sequential Recommendation

Sequential recommendation models are primarily optimized to distinguish positive samples from negative ones during training in which negative sampling serves as an essential component in learning the evolving user preferences through historical records. Except for randomly sampling negative samples from a uniformly distributed subset, many delicate methods have been proposed to mine negative samples with high quality. However, due to the inherent randomness of negative sampling, false negative samples are inevitably collected in model training. Current strategies mainly focus on removing such false negative samples, which leads to overlooking potential user interests, lack of recommendation diversity, less model robustness, and suffering from exposure bias. To this end, we propose a novel method that can Utilize False Negative samples for sequential Recommendation (UFNRec) to improve model performance. We first devise a simple strategy to extract false negative samples and then transfer these samples to positive samples in the following training process. Furthermore, we construct a teacher model to provide soft labels for false negative samples and design a consistency loss to regularize the predictions of these samples from the student model and the teacher model. To the best of our knowledge, this is the first work to utilize false negative samples instead of simply removing them for the sequential recommendation. Experiments on three benchmark public datasets are conducted using three widely applied SOTA models. The experiment results demonstrate that our proposed UFNRec can effectively draw information from false negative samples and further improve the performance of SOTA models. The code is available at https://github.com/UFNRec-code/UFNRec.

==> 5-Results.tex <==
\section{Analysis and Discussion}\label{sec:results}
% We have demonstrated the impressive performance of our proposed simple XXX on four backbones and four datasets.
% In this section, we conduct extensive experiments to analyze XXX from different views. 
% For convenience, related experiments are performed on the \textit{SASRec} backbone and \textit{Beauty} dataset. 
% More specifically, we mainly focus on: \textbf{1)} the influence of each operation (\textit{Ablation Study}), \textbf{2)} the effect of some important hyper-parameters (\textit{Hyper-Parameter Analysis}), 
% \textbf{3)} the analysis of training process and cost time (\textit{Training and Cost Analysis})

% \subsection{Ablation Study}
% \input{Table/table_ablation}
% As illustrated in Table~\ref{tb_ablation}, we conduct ablation study to explore the influence of two essential operations mentioned in Section~\ref{sec:method}, i.e., fake negative reversing and consistency regularization.

% \textbf{Fake Negative Reversing.} As shown in Table~\ref{tb_ablation}, the fake negative reversing method contributes significant improvement over the backbone \textit{SASRec} with a range of 1.87\% to 3.47\%, which further concludes that such fake negative samples are actually potential positive samples and false negative can perturb model performance. Compared with the consistency regularization, the fake negative reversing method approximately brings more improvement to the final results, which indicates that the quality of samples is extremely essential and our method can mitigate the incompatibility between the sampling process and the ground truth to some extent.

% \textbf{Fake Negative Consistency Regularization.} To only observe the effect of the consistency regularization objective, we maintain the fake negative mining process expect reversing, which means fake negative samples will not reverse to positive samples during train but still apply consistency training objective. Table~\ref{tb_ablation} shows that 

% \subsection{Hyper-Parameter Analysis}
%  In this part, we mainly analyze the influence of several critical hyper-parameters, including $\alpha$ in Equation~\ref{func:final_loss}, $d$ in Equation~\ref{func:tea_update}, the record time $m$ to reverse sample and batch size.

% \textbf{The Effect of $\alpha$.}
% \input{Table/MCR_parameter_l}
% Table~\ref{tb_parameter_alpha} shows the performance of different $\alpha$ values. 
% Since the combinations of the ($\alpha$, $d$, $m$) grid are complicated, we temporarily fix the decay rate $d=0.99$ and the epoch time to reverse $m=5$ to only analyze the effect of $\alpha$ for final loss.
% As shown in Table~\ref{tb_parameter_alpha}, only with a small value of $\alpha$, the consistency loss can achieve significant improvement.
% The performance improvement continuously increases along with the increase of $\alpha$, and achieves the best result at $\alpha=0.2$.
% These experiment results further prove that the consistency regularization of the above teacher-student framework on the fake negative samples is very powerful even when applying only a small value of $\alpha$ for the final loss during the training process.
% With a continuously increase of $\alpha$, the performance improvement start to decrease (e.g., $\alpha=0.2$ v.s.,$\alpha=0.4$), since the  excessive emphasis on the consistency of outputs from teacher-student framework dilutes the original objective to some extent.


% \textbf{The Effect of $d$.}
% \input{Table/MCR_parameter_d}

% \textbf{The Effect of $m$.}

% \input{Table/reverse_m}


% \textbf{The Effect of Batch Size.}
% \input{Table/Batchsize}



% \subsection{Training and Cost Analysis}


==> 6-Discussion.tex <==
\section{Discussion}


==> Table/Batchsize.tex <==

\begin{table}[]
\caption{The influence of batch size.}
\begin{tabular}{llllll}
\toprule
Metrics  & 32     & 64     & 128    & 256    & 512    \\
  \hline
HR@5                             & 0.3520 & 0.3743 & 0.3978 & 0.3940 & 0.3873 \\
HR@10                            & 0.4463 & 0.4745 & 0.4953 & 0.4913 & 0.4812 \\
HR@20                            & 0.5676 & 0.5888 & 0.6079 & 0.6001 & 0.5868 \\
NDCG@5                           & 0.2675 & 0.2877 & 0.3125 & 0.3089 & 0.3009 \\
NDCG@10                          & 0.2980 & 0.3199 & 0.3439 & 0.3403 & 0.3313 \\
NDCG@20                          & 0.3287 & 0.3489 & 0.3723 & 0.3678 & 0.3579\\
 \bottomrule
\end{tabular}
\label{tb_batchsize}
\end{table}

==> Table/MCR_parameter_d.tex <==
\begin{table}[]
\caption{The influence of parameter d, with fixed $\alpha$=0.3}
\begin{tabular}{lllll}
\toprule
Metrics  & 0.9    & 0.99   & 0.995  & 0.999  \\
\hline
HR@5                                & 0.3971 & 0.3964 & 0.3982 & 0.3978 \\
HR@10                               & 0.4918 & 0.4946 & 0.4946 & 0.4953 \\
HR@20                               & 0.6008 & 0.6056 & 0.6053 & 0.6079 \\
NDCG@5                              & 0.3085 & 0.3090 & 0.3120 & 0.3125 \\
NDCG@10                             & 0.3390 & 0.3408 & 0.3433 & 0.3439 \\
NDCG@20                             & 0.3665 & 0.3688 & 0.3712 & 0.3723
\\
 \bottomrule
\end{tabular}
\label{tb_parameter_d}
\end{table}

==> Table/MCR_parameter_l.tex <==
\begin{table}[]
\caption{The influence of parameter $\alpha$, with fixed d=0.99}
\begin{tabular}{lllll}
\toprule
Metrics & 0.1    & 0.2    & 0.3    & 0.4    \\
\hline
HR@5                                & 0.3923 & 0.3924 & 0.3964 & 0.3945 \\
HR@10                               & 0.4899 & 0.4957 & 0.4946 & 0.4925 \\
HR@20                               & 0.6013 & 0.6024 & 0.6056 & 0.6028 \\
NDCG@5                              & 0.3064 & 0.3068 & 0.3090 & 0.3076 \\
NDCG@10                             & 0.3379 & 0.3401 & 0.3408 & 0.3393 \\
NDCG@20                             & 0.3660 & 0.3671 & 0.3688 & 0.3672
\\
 \bottomrule
\end{tabular}
\label{tb_parameter_alpha}
\end{table}

==> Table/reverse_m.tex <==
\begin{table}[]
\caption{The reversing parameter m.}
\begin{tabular}{llllllll}
\toprule
& SASRec & m=2    & m=3    & m=4    & m=5    & m=6    \\
\hline
HR@5    & 0.3785 & 0.3655 & 0.383  & 0.3867 & 0.3903 & 0.3788 \\
HR@10   & 0.4765 & 0.4668 & 0.4873 & 0.4843 & 0.4872 & 0.4751 \\
HR@20   & 0.5891 & 0.5798 & 0.5976 & 0.6003 & 0.6001 & 0.5821 \\
NDCG@5  & 0.2942 & 0.2783 & 0.2943 & 0.3004 & 0.3044 & 0.2941 \\
NDCG@10 & 0.3258 & 0.3109 & 0.3278 & 0.3318 & 0.3356 & 0.3252 \\
NDCG@20 & 0.3543 & 0.3395 & 0.3556 & 0.3611 & 0.364  & 0.3522 \\
\bottomrule
\end{tabular}
\end{table}
